User-Customizable Transpilation of Scripting Languages

A transpiler converts code from one programming language to another. Many practical uses of transpilers require the user to be able to guide or customize the program produced from a given input program. This customizability is important for satisfying many application-specific goals for the produced code such as ensuring performance, readability, maintainability, compatibility, and so on. Conventional transpilers are deterministic rule-driven systems often written without offering customizability per user and per program. Recent advances in transpilers based on neural networks offer some customizability to users, e.g. through interactive prompts, but they are still difficult to precisely control the production of a desired output. Both conventional and neural transpilation also suffer from the "last mile" problem: they produce correct code on average, i.e., on most parts of a given program, but not necessarily for all parts of it. We propose a new transpilation approach that offers fine-grained customizability and reusability of transpilation rules created by others, without burdening the user to understand the global semantics of the given source program. Our approach is mostly automatic and incremental, i.e., constructs translation rules needed to transpile the given program as per the user's guidance piece-by-piece. We implement the transpiler as a tool called DuoGlot, which translates Python to Javascript programs, and evaluate it on the popular GeeksForGeeks benchmarks. DuoGlot achieves 90% translation accuracy and so it outperforms all existing translators, while it produces readable code. We evaluate DuoGlot on two additional benchmarks, containing more challenging and longer programs, and similarly observe improved accuracy.

==> figtabs/fig-certainlycore.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{imgs/certainlyperp.png}
 %
    \caption{Implementation of \tool.}
    \label{fig:certainlycore}
\end{figure}

==> figtabs/fig-motivateflowex.tex <==
\begin{figure}[!htbp]
    \centering
    \begin{tabular}{@{}c@{}}
        \includegraphics[width=\textwidth]{imgs/motiv-incremental.png}\\
 %
 %
 %
 %
        \small  \\
    \end{tabular}
    \caption{An example of translating a \pylang function to \jslang given some unit tests.  At the beginning, the incremental translator fails because there's no rule to translate list comprehension. Then the user provides code snippets for translating list comprehension. A translation rule will be automatically extracted from the code snippets and added to \tool. Then the translator will get candidate translations and run unit tests. If the unit tests fails, failure information is used to guide \tool's candidate search. After 13 retries, \tool finds a candidate that produce the same outputs as the source program on unit tests and returns candidate 13 as the result. }
    \label{fig:motivateflowex}
\end{figure}


==> figtabs/fig-motivatesearch.tex <==
\begin{figure}[!htbp]
    \centering
    \begin{tabular}{@{}c@{}}
            \includegraphics[width=0.70\textwidth]{imgs/motiv-select1.png}\\ \includegraphics[width=0.70\textwidth]{imgs/motiv-select2.png}\\
        \small  \\
    \end{tabular}
    \caption{Examples of \pylang to \jslang translation showing the semantic-mismatch problem. The first example is translating \texttt{int(x)} and the second example is translating \texttt{if x in y}. On the right-side is the set diagram of input space. Intersections between circles are the part of the input space that they have the same outcome. Black dots are some example inputs in those sub-spaces. A correct or good translation depends on possible inputs. }
    \label{fig:motivatesearch}
\end{figure}


==> figtabs/fig-rulecategory.tex <==


\begin{myverbbox}[\scriptsize]{\baseverb}
### Python:
a = 5

### JavaScript: 
a = 5
\end{myverbbox}

\begin{myverbbox}[\scriptsize]{\simpleverb}
### Python:
not x
not y == 0

### JavaScript: 
!(x)
!(y === 0)
\end{myverbbox}

\begin{myverbbox}[\scriptsize]{\mediumverb}
### Python:
for i in range(1,x,2):
  ...

### JavaScript: 
for (let i = 1; i < x; i += 2) {
  ...
}
\end{myverbbox}

\begin{myverbbox}[\scriptsize]{\mediumverbaaaa}
### Python:
"hello".isupper()

### JavaScript: 
"hello" === "hello".toUpperCase()
\end{myverbbox}

\begin{myverbbox}[\scriptsize]{\mediumverbbbbb}
### Python:
list1.remove("bob")

### JavaScript: 
list1.splice(list1.indexOf("bob"), 1)
\end{myverbbox}


\begin{myverbbox}[\scriptsize]{\complexverb}
### Python:
{x["id"]:x for x in xs}

### JavaScript: 
Array.from(xs)
  .map((x) => [x["id"], x])
  .reduce(
    (a, b) => (a[b[0]] = b[1], a),
    {});
\end{myverbbox}

\begin{table}[!htbp]
    \centering
 %
 %
 %
 %
    
    \begin{tabular}{|@{}l@{}|@{}c@{}|@{}l@{}|}
    \hline 
    \mycentered{Category} & \mycentered{Example Rule} & \mycentered{Translation} \\
    \hline 
    \mycentered{Initial} &
    \mycentered{\includegraphics[width=0.5\linewidth]{imgs/base1.png}} &\mycentered{\baseverb}\\
    \hline 
    \mycentered{Simple} &
    \mycentered{\includegraphics[width=0.5\linewidth]{imgs/simple1.png}} &\mycentered{\simpleverb}\\
    \hline 
    \mycentered{Simple} &
    \mycentered{\includegraphics[width=0.5\linewidth]{imgs/medium2.png}} & \mycentered{\mediumverbaaaa}\\
    \hline 
    \mycentered{Medium} &
    \mycentered{\includegraphics[width=0.5\linewidth]{imgs/medium3.png}} & \mycentered{\mediumverbbbbb}\\
    \hline 
    \mycentered{Complex} &
    \mycentered{\includegraphics[width=0.5\linewidth]{imgs/complex1.png}} & \mycentered{\complexverb}\\
    \hline 
    \end{tabular}
    \caption{Example of rules in "Simple", "Medium" and "Complex" category}
    \label{tbl:rulecategory}
\end{table}



==> figtabs/fig-rulecountperf.tex <==
\begin{figure}[ht]
    \centering
    \begin{tikzpicture}[]
    \begin{axis}[
    table/col sep=comma,
 %
    xticklabel style={rotate=45, anchor=near xticklabel},
    xmin=0,
    xmax=150,
    xlabel={Number of rules},
    ylabel={Accuracy (\%)},
    ymin=0,
    ymax=1, 
    max space between ticks=20,
    stack plots=x,
    area style,
    ]
    \addplot table [mark=none,x=rulecount,y=accuracy] {\loadedtable}
    \closedcycle;
 %
 %
 %
 %
    \end{axis}
    \end{tikzpicture}
    \caption{The percentage of benchmarks from \gfgbenchmark translated correctly by \tool as a function of the number of rules.}
    \label{fig:rulecountperf}
\end{figure}
